Letter of Intent: A New QCD facility at the M2 beam line of the CERN SPS (COMPASS++/AMBER)

A New QCD facility at the M2 beam line of the CERN SPS COMPASS++/AMBER

==> Makefile <==
MAINFILE=loi2017
TEXFILES=$(wildcard *.tex) \
         $(wildcard ./*/*.tex) \
         $(wildcard ./*/*/*.tex)
INCFILES=$(wildcard *.tex)
AUXFILES=$(patsubst %.tex, %.aux, $(INCFILES)) 
#AUXFILES=$(wildcard *.aux)
BIBFILES=$(wildcard ./bib/*.bib)
BBLFILES=$(patsubst %.tex, %.bbl, $(INCFILES)) 
#BBLFILES=$(MAINFILE).bbl
FIGFILES=$(wildcard ./fig/*.pdf) \
         $(wildcard ./fig/*.jpg) \
         $(wildcard ./fig/*.png) 

export TEXINPUTS=.:./sty:./tex:./bib:$TEXINPUTS:
export BSTINPUTS=.:./sty:$BSTINPUTS:
export BIBINPUTS=.:./bib:$BIBINPUTS:

all:	$(MAINFILE).pdf

test:
	@echo ``TEXFILES:'' $(TEXFILES)
	@echo ``INCFILES:'' $(INCFILES)
	@echo ``AUXFILES:'' $(AUXFILES)
	@echo ``BIBFILES:'' $(BIBFILES)
	@echo ``BBLFILES:'' $(BBLFILES)
	@echo ``FIGFILES:'' $(FIGFILES)

emacs:
	emacs $(TEXFILES) &

$(MAINFILE).pdf: $(MAINFILE).tex $(FIGFILES) $(TEXFILES) $(BBLFILES)
	@echo "============ Main LaTeX pass ============"
	-pdflatex --shell-escape $(MAINFILE) 
	pdflatex --shell-escape $(MAINFILE) 
#	pdflatex --shell-escape $(MAINFILE) 

%.bbl:	%.aux 
	@echo "============ BibTeX pass ============"
	-bibtex $(patsubst %.aux,%,$^)

#%.bbl: %.tex $(BIBFILES)
#	-bibtex $(MAINFILE)

%.aux: 	%.tex
	@echo "============ TEX -> AUX pass for" $@ "============" 
	-pdflatex --shell-escape $(MAINFILE) 

clean:
	@echo "============ Cleaning ============" 
	-rm -rf *.aux *.blg *.bbl *.log *.out *.toc *.lof *.brf

distclean: clean
	@echo "============ Thorough cleaning ============" 
	-rm -rf $(MAINFILE).pdf *~

.PRECIOUS: %.bbl %.aux

.PHONY: clean distclean test all emacs



==> tex/AuthorsCOMPASS2018.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 2018_auththorlist.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Dear all,
%
%in these years i received a (small) amount of money from my univeristy
%(outside the big money from INFN) for my research. i have always spent these money for compass and in particular recently to pay a short contract for bakur. in order to justify how i spent these money, i need that in one of next compass papers (the earliest the best) a sentence like:
%
%"This research has been funded in part by Universita' del Piemonte Orientale,Italy."
%
%i sincerely hope this is not a problem.
%
%kind regards,
%
%        daniele
%
\section*{The COMPASS Collaboration}
\label{app:collab}
\renewcommand\labelenumi{\textsuperscript{\theenumi}~}
\renewcommand\theenumi{\arabic{enumi}}
\begin{flushleft}
R.~Akhunzyanov\Irefn{dubna}, % phd
M.G.~Alexeev\Irefn{turin_u},
G.D.~Alexeev\Irefn{dubna}, %1
A.~Amoroso\Irefnn{turin_u}{turin_i},
V.~Andrieux\Irefnn{illinois}{saclay},
N.V.~Anfimov\Irefn{dubna}, %2
V.~Anosov\Irefn{dubna}, %3
A.~Antoshkin\Irefn{dubna}, % phd
K.~Augsten\Irefnn{dubna}{praguectu}, %prague
W.~Augustyniak\Irefn{warsaw},
C.D.R.~Azevedo\Irefn{aveiro},
B.~Bade{\l}ek\Irefn{warsawu},
F.~Balestra\Irefnn{turin_u}{turin_i},
M.~Ball\Irefn{bonniskp},
J.~Barth\Irefn{bonnpi},
R.~Beck\Irefn{bonniskp},
Y.~Bedfer\Irefn{saclay},
J.~Berenguer Antequera\Irefnn{turin_u}{turin_i},
J.~Bernhard\Irefnn{mainz}{cern},
E.~R.~Bielert\Irefn{cern},
M.~Bodlak\Irefn{praguecu},
P.~Bordalo\Irefn{lisbon}\Aref{a},
F.~Bradamante\Irefnn{triest_u}{triest_i},
A.~Bressan\Irefnn{triest_u}{triest_i},
M.~B\"uchele\Irefn{freiburg},
V.E.~Burtsev\Irefn{tomsk},
W.-C.~Chang\Irefn{taipei},
C.~Chatterjee\Irefn{calcutta},
M.~Chiosso\Irefnn{turin_u}{turin_i},
A.G.~Chumakov\Irefn{tomsk},
S.-U.~Chung\Irefn{munichtu}\Aref{b},
A.~Cicuttin\Irefn{triest_i}\Aref{ictp},
P.~Correia\Irefn{lisbon};
M.L.~Crespo\Irefn{triest_i}\Aref{ictp},
S.~Dalla Torre\Irefn{triest_i},
S.S.~Dasgupta\Irefn{calcutta},
S.~Dasgupta\Irefnn{triest_u}{triest_i},
I.~Denisenko\Irefn{dubna},
O.Yu.~Denisov\Irefn{turin_i}, %\CorAuth,
L.~Dhara\Irefn{calcutta},
S.V.~Donskov\Irefn{protvino},
N.~Doshita\Irefn{yamagata},
Ch.~Dreisbach\Irefn{munichtu},
W.~D\"unnweber\Arefs{r},
R.R.~Dusaev\Irefn{tomsk},
M.~Dziewiecki\Irefn{warsawtu},
A.~Efremov\Irefn{dubna}, %4
P.D.~Eversheim\Irefn{bonniskp},
M.~Faessler\Arefs{r},
A.~Ferrero\Irefn{saclay},
M.~Finger\Irefn{praguecu},
M.~Finger~jr.\Irefn{praguecu},
H.~Fischer\Irefn{freiburg},
C.~Franco\Irefn{lisbon},
N.~du~Fresne~von~Hohenesche\Irefnn{mainz}{cern},
J.M.~Friedrich\Irefn{munichtu}, %\CorAuth,
V.~Frolov\Irefnn{dubna}{cern},   %5
A.~Futch\Irefn{illinois},
F.~Gautheron\Irefnn{bochum}{illinois},
O.P.~Gavrichtchouk\Irefn{dubna}, %6
S.~Gerassimov\Irefnn{moscowlpi}{munichtu},
J.~Giarra\Irefn{mainz},
I.~Gnesi\Irefnn{turin_u}{turin_i},
M.~Gorzellik\Irefn{freiburg},
A.~Grasso\Irefnn{turin_u}{turin_i},
A.~Gridin\Irefn{dubna},
M.~Grosse Perdekamp\Irefn{illinois},
B.~Grube\Irefn{munichtu},
R.I.~Gushterski\Irefn{dubna},
A.~Guskov\Irefn{dubna}, %7
D.~Hahne\Irefn{bonnpi},
G.~Hamar\Irefn{triest_i},
D.~von~Harrach\Irefn{mainz},
R.~Heitz\Irefn{illinois},
F.~Herrmann\Irefn{freiburg},
N.~Horikawa\Irefn{nagoya}\Aref{d},
N.~d'Hose\Irefn{saclay},
C.-Y.~Hsieh\Irefn{taipei}\Aref{x},
S.~Huber\Irefn{munichtu},
S.~Ishimoto\Irefn{yamagata}\Aref{e},
A.~Ivanov\Irefnn{turin_u}{turin_i},
Yu.~Ivanshin\Irefn{dubna},
M.~Jandek\Irefn{praguecu},
T.~Iwata\Irefn{yamagata},
V.~Jary\Irefn{praguectu},
R.~Joosten\Irefn{bonniskp},
P.~J\"org\Irefn{freiburg},
K.~Juraskova\Irefn{praguectu},
F.~Kaspar\Irefn{munichtu},
E.~Kabu\ss\Irefn{mainz},
A.~Kerbizi\Irefnn{triest_u}{triest_i},
B.~Ketzer\Irefn{bonniskp},%\Aref{f},
G.V.~Khaustov\Irefn{protvino},
Yu.A.~Khokhlov\Irefn{protvino}%\Aref{v},
Yu.~Kisselev\Irefn{dubna}, %9
F.~Klein\Irefn{bonnpi},
J.H.~Koivuniemi\Irefnn{bochum}{illinois},
V.N.~Kolosov\Irefn{protvino},
K.~Kondo\Irefn{yamagata},
I.~Konorov\Irefnn{moscowlpi}{munichtu},
V.F.~Konstantinov\Irefn{protvino},
A.~Koval\Irefn{warsaw},
A.M.~Kotzinian\Irefn{turin_i}\Aref{yerevan},
O.M.~Kouznetsov\Irefn{dubna}, %10
Z.~Kral\Irefn{praguectu},
M.~Kr\"amer\Irefn{munichtu},
F.~Krinner\Irefn{munichtu},
Y.~Kulinich\Irefn{illinois},
F.~Kunne\Irefn{saclay},
K.~Kurek\Irefn{warsaw},
R.P.~Kurjata\Irefn{warsawtu},
I.I.~Kuznetsov\Irefn{tomsk},
A.~Kveton\Irefn{praguectu},
E.A.~Levchenko\Irefn{tomsk},
S.~Levorato\Irefn{triest_i},
Y.-S.~Lian\Irefn{taipei}\Aref{y},
P.-J.~Lin\Irefn{saclay},
J.~Lichtenstadt\Irefn{telaviv},
R.~Longo\Irefnn{turin_u}{turin_i},
V.E.~Lyubovitskij\Irefn{tomsk}\Aref{regen},
A.~Maggiora\Irefn{turin_i},
A.~Magnon\Irefn{illinois},
N.~Makins\Irefn{illinois},
N.~Makke\Irefn{triest_i}\Aref{ictp},
G.K.~Mallot\Irefn{cern},
S.A.~Mamon\Irefn{tomsk},
B.~Marianski\Irefn{warsaw},
A.~Martin\Irefnn{triest_u}{triest_i},
J.~Marzec\Irefn{warsawtu},
J.~Matou{\v s}ek\Irefnnn{triest_u}{triest_i}{praguecu},
H.~Matsuda\Irefn{yamagata},
G.~Mattson\Irefn{illinois},
G.V.~Meshcheryakov\Irefn{dubna}, %12
M.~Meyer\Irefnn{illinois}{saclay},
W.~Meyer\Irefn{bochum},
Yu.V.~Mikhailov\Irefn{protvino},
M.~Mikhasenko\Irefn{bonniskp},
E.~Mitrofanov\Irefn{dubna},  % phd
N.~Mitrofanov\Irefn{dubna},  % phd
Y.~Miyachi\Irefn{yamagata},
A.~Moretti\Irefn{triest_u},
C.~Na\"im\Irefn{saclay},
A.~Nagaytsev\Irefn{dubna}, %13
D.~Neyret\Irefn{saclay},
J.~Nov{\'y}\Irefnn{praguectu}{cern},
W.-D.~Nowak\Irefn{mainz},
G.~Nukazuka\Irefn{yamagata},
A.S.~Nunes\Irefn{lisbon},
A.G.~Olshevsky\Irefn{dubna}, %14
I.~Orlov\Irefn{dubna}, % phd
M.~Ostrick\Irefn{mainz},
D.~Panzieri\Irefn{turin_i}\Aref{turin_p},
B.~Parsamyan\Irefnn{turin_u}{turin_i},
S.~Paul\Irefn{munichtu},
J.-C.~Peng\Irefn{illinois},
F.~Pereira\Irefn{aveiro},
M.~Pe{\v s}ek\Irefn{praguecu},
M.~Pe{\v s}kov\'a\Irefn{praguecu},
D.V.~Peshekhonov\Irefn{dubna}, %15
N.~Pierre\Irefnn{mainz}{saclay},
S.~Platchkov\Irefn{saclay},
J.~Pochodzalla\Irefn{mainz},
V.A.~Polyakov\Irefn{protvino},
J.~Pretz\Irefn{bonnpi}\Aref{h},
M.~Quaresma\Irefn{lisbon},
C.~Quintans\Irefn{lisbon},
S.~Ramos\Irefn{lisbon}\Aref{a},
C.~Regali\Irefn{freiburg},
G.~Reicherz\Irefn{bochum},
C.~Riedl\Irefn{illinois},
D.I.~Ryabchikov\Irefnn{protvino}{munichtu}, %\Aref{v},
A.~Rybnikov\Irefn{dubna}, % phd
A.~Rychter\Irefn{warsawtu},
R.~Salac\Irefn{praguectu},
V.D.~Samoylenko\Irefn{protvino},
A.~Sandacz\Irefn{warsaw},
S.~Sarkar\Irefn{calcutta},
I.A.~Savin\Irefn{dubna}, %16
G.~Sbrizzai\Irefnn{triest_u}{triest_i},
H.~Schmieden\Irefn{bonnpi},
E.~Seder\Irefn{saclay},
A.~Selyunin\Irefn{dubna}, % phd
L.~Silva\Irefn{lisbon},
L.~Sinha\Irefn{calcutta},
S.~Sirtl\Irefn{freiburg},
M.~Slunecka\Irefn{dubna}, %17
J.~Smolik\Irefn{dubna}, %18
A.~Srnka\Irefn{brno},
D.~Steffen\Irefnn{cern}{munichtu},
M.~Stolarski\Irefn{lisbon},
O.~Subrt\Irefnn{cern}{praguectu},
M.~Sulc\Irefn{liberec},
H.~Suzuki\Irefn{yamagata}\Aref{d},
A.~Szabelski\Irefnnn{triest_u}{triest_i}{warsaw} %also {triest_i}
T.~Szameitat\Irefn{freiburg},
P.~Sznajder\Irefn{warsaw},
M.~Tasevsky\Irefn{dubna}, %19
S.~Tessaro\Irefn{triest_i},
F.~Tessarotto\Irefn{triest_i},
A.~Thiel\Irefn{bonniskp},
J.~Tomsa\Irefn{praguecu},
F.~Tosello\Irefn{turin_i},
V.~Tskhay\Irefn{moscowlpi},
S.~Uhl\Irefn{munichtu},
B.I.~Vasilishin\Irefn{tomsk},
A.~Vauth\Irefn{cern},
B.M.~Veit\Irefn{mainz},
J.~Veloso\Irefn{aveiro},
A.~Vidon\Irefn{saclay},
M.~Virius\Irefn{praguectu},
M.~Wagner\Irefn{bonniskp},
S.~Wallner\Irefn{munichtu},
M.~Wilfert\Irefn{mainz},
K.~Zaremba\Irefn{warsawtu},
P.~Zavada\Irefn{dubna}, %20
M.~Zavertyaev\Irefn{moscowlpi},
E.~Zemlyanichkina\Irefn{dubna}, %21
Y.~Zhao\Irefn{triest_i},
N.~Zhuravlev\Irefn{dubna}, %22
M.~Ziembicki\Irefn{warsawtu}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% institutes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Authlist}
\item \Idef{aveiro}{University of Aveiro, Dept.\ of Physics, 3810-193 Aveiro, Portugal}
\item \Idef{bochum}{Universit\"at Bochum, Institut f\"ur Experimentalphysik, 44780 Bochum, Germany}
\item \Idef{bonniskp}{Universit\"at Bonn, Helmholtz-Institut f\"ur  Strahlen- und Kernphysik, 53115 Bonn, Germany}
\item \Idef{bonnpi}{Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany}
\item \Idef{brno}{Institute of Scientific Instruments, AS CR, 61264 Brno, Czech Republic}
\item \Idef{calcutta}{Matrivani Institute of Experimental Research \& Education, Calcutta-700 030, India}
\item \Idef{dubna}{Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia}
\item \Idef{freiburg}{Universit\"at Freiburg, Physikalisches Institut, 79104 Freiburg, Germany}
\item \Idef{cern}{CERN, 1211 Geneva 23, Switzerland}
\item \Idef{liberec}{Technical University in Liberec, 46117 Liberec, Czech Republic}
\item \Idef{lisbon}{LIP, 1000-149 Lisbon, Portugal}
\item \Idef{mainz}{Universit\"at Mainz, Institut f\"ur Kernphysik, 55099 Mainz, Germany}
\item \Idef{miyazaki}{University of Miyazaki, Miyazaki 889-2192, Japan}
\item \Idef{moscowlpi}{Lebedev Physical Institute, 119991 Moscow, Russia}
\item \Idef{munichtu}{Technische Universit\"at M\"unchen, Physik Dept., 85748 Garching, Germany}
\item \Idef{nagoya}{Nagoya University, 464 Nagoya, Japan}
\item \Idef{praguecu}{Charles University in Prague, Faculty of Mathematics and Physics, 18000 Prague, Czech Republic}
\item \Idef{praguectu}{Czech Technical University in Prague, 16636 Prague, Czech Republic}
\item \Idef{protvino}{State Scientific Center Institute for High Energy Physics of National Research Center `Kurchatov Institute', 142281 Protvino, Russia}
\item \Idef{saclay}{IRFU, CEA, Universit\'e Paris-Saclay, 91191 Gif-sur-Yvette, France}
\item \Idef{taipei}{Academia Sinica, Institute of Physics, Taipei 11529, Taiwan}
\item \Idef{telaviv}{Tel Aviv University, School of Physics and Astronomy, 69978 Tel Aviv, Israel}
\item \Idef{triest_u}{University of Trieste, Dept.\ of Physics, 34127 Trieste, Italy}
\item \Idef{triest_i}{Trieste Section of INFN, 34127 Trieste, Italy}
\item \Idef{turin_u}{University of Turin, Dept.\ of Physics, 10125 Turin, Italy}
\item \Idef{turin_i}{Torino Section of INFN, 10125 Turin, Italy}
\item \Idef{tomsk}{Tomsk Polytechnic University,634050 Tomsk, Russia}
\item \Idef{illinois}{University of Illinois at Urbana-Champaign, Dept.\ of Physics, Urbana, IL 61801-3080, USA}
\item \Idef{warsaw}{National Centre for Nuclear Research, 00-681 Warsaw, Poland}
\item \Idef{warsawu}{University of Warsaw, Faculty of Physics, 02-093 Warsaw, Poland}
\item \Idef{warsawtu}{Warsaw University of Technology, Institute of Radioelectronics, 00-665 Warsaw, Poland }
\item \Idef{yamagata}{Yamagata University, Yamagata 992-8510, Japan }
\end{Authlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Notes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\theenumi{\alph{enumi}}
\begin{Authlist}
%\item [{\makebox[2mm][l]{\textsuperscript{\#}}}] Corresponding authors
%\item [{\makebox[2mm][l]{\textsuperscript{*}}}] Deceased
\item \Adef{a}{Also at Instituto Superior T\'ecnico, Universidade de Lisboa, Lisbon, Portugal}
\item \Adef{b}{Also at Dept.\ of Physics, Pusan National University, Busan 609-735, Republic of Korea and at Physics Dept., Brookhaven National Laboratory, Upton, NY 11973, USA}
\item \Adef{ictp}{Also at Abdus Salam ICTP, 34151 Trieste, Italy}
\item \Adef{r}{Supported by the DFG cluster of excellence `Origin and Structure of the Universe' (www.universe-cluster.de) (Germany)}
%\item \Adef{p2i}{Supported by the Laboratoire d'excellence P2IO (France)}
%\item \Adef{fuchey_adr}{Present address:  University of Connecticut, Storrs, Connecticut 06269, US}
%\item \Adef{joerg_adr}{Present address: Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany}
\item \Adef{d}{Also at Chubu University, Kasugai, Aichi 487-8501, Japan}
\item \Adef{x}{Also at Dept.\ of Physics, National Central University, 300 Jhongda Road, Jhongli 32001, Taiwan}
\item \Adef{e}{Also at KEK, 1-1 Oho, Tsukuba, Ibaraki 305-0801, Japan}
\item \Adef{g}{Also at Moscow Institute of Physics and Technology, Moscow Region, 141700, Russia}
%\item \Adef{v}{Supported by Presidential Grant NSh--999.2014.2 (Russia)}
\item \Adef{h}{Present address: RWTH Aachen University, III.\ Physikalisches Institut, 52056 Aachen, Germany}
\item \Adef{yerevan}{Also at Yerevan Physics Institute, Alikhanian Br. Street, Yerevan, Armenia, 0036}
\item \Adef{y}{Also at Dept.\ of Physics, National Kaohsiung Normal University, Kaohsiung County 824, Taiwan}
\item \Adef{regen}{Also at Institut f\"ur Theoretische Physik, Universit\"at T\"ubingen, 72076 T\"ubingen, Germany}
%\item \Adef{infn}{Also at \ref{LItriest_i})}
\item \Adef{turin_p}{Also at University of Eastern Piedmont, 15100 Alessandria, Italy}
%\item \Adef{i}{Present address: Uppsala University, Box 516, 75120 Uppsala, Sweden}
%\item \Adef{c}{    Supported by the DFG Research Training Group Programmes 1102 and 2044 (Germany)} %mail Horst Fischer 20/09/2016 11:08
%
% support institutes
%
%\item \Adef{l}{    Supported by BMBF - Bundesministerium f\"ur Bildung und Forschung (Germany)}
%\item \Adef{s}{    Supported by FP7, HadronPhysics3, Grant 283286 (European Union)}
%\item \Adef{m}{    Supported by MEYS, Grant LG13031 (Czech Republic)}
%\item \Adef{n}{    Supported by B.Sen fund (India)}
%\item \Adef{o}{    Supported by CERN-RFBR Grant 12-02-91500}
%\item \Adef{p}{\raggedright 
%                   Supported by FCT - Funda\c{c}\~{a}o para a Ci\^{e}ncia e Tecnologia, COMPETE and QREN, Grants CERN/FP 116376/2010, 123600/2011 
%                   and CERN/FIS-NUC/0017/2015 (Portugal)}
%\item \Adef{q}{    Supported by MEXT and JSPS, Grants 18002006, 20540299, 18540281 and 26247032, the Daiko and Yamada Foundations (Japan)}
%\item \Adef{tw}{   Supported by the Ministry of Science and Technology (Taiwan)}
%\item \Adef{t}{    Supported by the Israel Academy of Sciences and Humanities (Israel)}
%\item \Adef{nauka}{Supported by the Russian Federation  program ``Nauka'' (Contract No. 0.1764.GZB.2017) (Russia)}
%\item \Adef{nsf}{  Supported by the National Science Foundation, Grant no. PHY-1506416 (USA)}
%\item \Adef{u}{    Supported by NCN, Grant 2017/26/M/ST2/00498 (Poland)}
%
\end{Authlist}
%
%



==> tex/stdhad_spect_short.tex <==
\svnid{$Id: stdhad_spect_short.tex 4404 2018-10-08 18:17:46Z avauth $} 
\subsection{Spectroscopy with Low-Energy Antiprotons}
\label{sec:stdhad.spect}
COMPASS has studied the spectrum of light quarks with
unprecedented statistical precision, requiring the development of
novel analysis techniques in order to minimise the model bias when
interpreting the data. Using a high-energy pion or proton beam
scattering off a liquid hydrogen or solid nuclear targets, excited
states were produced in diffractive reactions which are dominated by
the exchange of a Pomeron in the $t$-channel
(\figref{fig:exp.production.diff}).    

Experiments employing the annihilation of antiprotons on protons or
neutrons provide a different and complementary access to excited
states of mesons and baryons, covering not only the light and strange
quark sector, but also the charmonium and possibly the bottomonium
region. The  M2 beam line can provide, with minimal modifications
compared to the present setup, a rather clean beam of antiprotons with
momenta between $12$ and $20\,\mathrm{GeV}$. According to preliminary
calculations, 
the intensity of antiprotons at the target is between $1.1\cdot
10^{7}$ and 
$1.8\cdot 10^{7}$ per pulse of $10^{13}$ protons on the production
target at momenta of $12$ and $20$~GeV, respectively, and is limited
by radiation protection issues. Employing a
$40$~cm long liquid hydrogen target, as for the measurements with a
pion beam, a luminosity of the order of  
$10^{30}\,\mathrm{cm}^{-2}\mathrm{s}^{-1}$ can be achieved. 

This opens
the possibility to use antiproton annihilations as a tool to study the
spectrum of charm and possibly also beauty hadrons. Especially the
production 
in association with a recoil particle allows states with spin-exotic
quantum numbers to be produced. This is the mode with the highest
discovery potential for states beyond the standard $q\overline{q}$
configuration, including states with explicit gluonic degrees of
freedom, i.e.\ hybrids and glueballs. According to model and lattice
calculations, the lightest charmonium hybrid is predicted at a mass
around $4.3\,\mathrm{GeV}$ with spin-exotic quantum numbers. Also the
lowest-mass  
glueball with spin-exotic quantum numbers, predicted at a mass between
$4$ and  $5\,\mathrm{GeV}$
is within the kinematic reach of this experiment. Other possible
measurements include the measurements of $\verline{p}p$ production
cross sections for $X,Y,Z$ states, which are vital for future
precision experiments employing antiproton annihilations like PANDA. 

The setup for these measurements will make use of the existing forward 
spectrometer, augmented by a powerful target
spectrometer to maximise the acceptance for exclusive measurements of
multi-particle final states. We are currently investigating several
options in this direction, including e.g.\ the use of parts of the
WASA spectrometer. 



==> tex/stdmuo_mup_setup.tex <==
\svnid{$Id: stdmuo_mup_setup.tex 4376 2018-09-11 09:50:37Z avauth $} 
\subsubsection{Experimental setup}
\label{sec:stdmuo.mup.setup}

The experimental setup uses the standard muon beam setup of COMPASS, but the target region will be modified as to accommodate an active hydrogen target, possibly an active SciFi target, and two silicon telescopes. Proton recoil measurement, muon measurement, and the trigger of this experiment are detailed in Sec.~\ref{sec:inst-mup}.






==> tex/stdmuo_sidis.tex <==
\svnid{$Id: stdmuo_sidis.tex 4404 2018-10-08 18:17:46Z avauth $} 
\subsection{Semi-inclusive Deep-Inelastic Scattering off transversely polarised deuteron}
\label{sec:stdmuo.sidis}

\subsubsection{Introduction}
In collinear QCD, when the transverse momentum of the partons is neglected, 
three parton distribution functions (PDFs) fully describe the nucleon at the 
twist-two level: the momentum distributions $f_1^q(x)$, the helicity distributions 
$g_1^q(x)$ and the transversity distributions $h_1^q(x)$ \cite{Mulders:1995dh}
where $x$ is the Bjorken variable. 
On the other hand, from the measured azimuthal asymmetries of hadrons 
produced in unpolarised semi-inclusive deep inelastic scattering (SIDIS) 
and Drell-Yan (DY) processes a sizeable transverse momentum of quarks was 
derived. 
Taking into account a finite intrinsic transverse momentum $k_T$, 
in total eight transverse momentum dependent (TMD) distribution functions 
are required to fully describe the nucleon at leading twist~\cite{Barone:2010zz,Aidala:2012mv,Avakian:2016rst}. 
Presently, PDFs that describe non-perturbative properties of hadrons are not 
yet calculable in QCD from first principles, but they can already be computed 
in lattice QCD. 
In the SIDIS cross section they appear convoluted with fragmentation 
functions (FFs)~\cite{Kotzinian:1994dv,Bacchetta:2006tn}, 
so that they can be extracted from the data.

Since transverse spin couples naturally to intrinsic transverse momentum, 
the resulting correlations are encoded in various transverse-momentum-dependent
parton distribution and fragmentation functions (FFs). 
Particularly interesting is therefore the measurement of the SIDIS 
cross section when the target nucleon is transversely polarised. 
In this case 8 different spin-dependent azimuthal modulations are expected, 
from which invaluable information on the TMD PDFs can be extracted.
In this domain the HERMES and the \compass collaborations have performed 
pioneering measurements and shown beyond any possible doubt the correctness 
of two most important recent conjectures:
\begin{itemize}
\item[-] The Sivers function: in a nucleon that is polarised
  transversely to its momentum the quark distribution is not
  left-right symmetric with respect to the plane defined by the
  directions of the nucleon spin and momentum.  This asymmetry of the
  distribution function is called the Sivers effect, and the
  asymmetric distribution is known as the Sivers distribution
  function~\cite{Sivers:1989cc}.
\item[-] The Collins function: the hadronisation of a transversely
  polarised quark is not left-right symmetric with respect to the
  plane defined by the quark momentum and the quark
  spin~\cite{Collins:1992kk}. This fact has been exploited to measure
  the quark transverse polarisation in a transversely polarised
  nucleon, namely the quark transversity PDF.
\end{itemize}
HERMES~\cite{Airapetian:2009ti} and
\compass~\cite{Adolph:2012sp,Adolph:2012sn,Adolph:2014fjw} are up to
now the only SIDIS experiments that have shown that both the Sivers
function and the Collins function are different from zero.
Independent evidence that the Collins effect is non zero has been
provided at the $e^+e^-$ colliders, by looking at the azimuthal
correlations of hadrons produced in opposite jets~\cite{Abe:2005zx,Osipenko:2008rv},  
so that global analyses using the SIDIS and the e+e- data could result in 
the extraction of the quark transversity PDF~\cite{Anselmino:2007fs,Efremov:2008vf}. 
The non zero results were obtained on proton targets. 
\compass has also measured transverse spin asymmetries using a deuteron 
target~\cite{Ageev:2006da}. 
The accuracy of the data is definitely inferior to that of the proton data, 
and the results where compatible with zero, hinting at possible cancellation 
between u and d quarks. 
More recently data have been collected at JLab on a $^3$He target, essentially 
transversely polarised neutrons: the measured asymmetries~\cite{Qian:2011py,Zhao:2014qvx}
are also compatible with zero, but the error bars are fairly large.
The \compass data are still today the only SIDIS data ever taken on a 
transversely polarised deuteron target and provide constraints on the 
d-quark contribution.  
We propose to perform a one-year measurement  scattering the M2 muon beam 
at 160 GeV/c momentum on a transversely polarised deuteron target, so that, 
combining the new deuteron data with the good precision proton data 
collected in the year 2010, the u- and d-distribution functions can be 
extracted from the SIDIS asymmetry data with comparable accuracies. 
This measurement was indeed proposed already in the original \compass proposal, 
but could not be performed in the early years of data taking due to the late 
delivery of the \compass polarised target magnet.

\subsubsection{The case for transversity}


In this section the case for the Collins asymmetry and the extraction of 
transversity for the u and d quarks will be detailed, but clearly all 
the spin dependent azimuthal modulations in the SIDIS cross section provide 
information on the nucleon PDFs and are of great interest. 
The measurement of the quark transversity distributions, which are defined 
in terms of the nucleon matrix element of the quark tensor current, is 
particularly important because it provides access to the quark tensor 
charges $\delta q$, which are given by the integral
\begin{eqnarray}
\delta q (Q^2)= \int_0^1 dx [h_1^q(x,Q^2)-h_1^{\bar{q}}(x,Q^2)
\end{eqnarray}
In a non-relativistic quark model, $h_1^q$ is equal to $g_1^q$, 
and $\delta q$ is 
equal to the valence quark contribution to the nucleon spin.  
The difference between hq1 and gq1 provides important constraints to any 
model of the nucleon. 
Knowing the quark tensor charges one can construct the isovector nucleon 
tensor charge  $g_T = \delta u- \delta d$, a fundamental property of the 
nucleon which, together with the vector and axial charge, characterizes 
the nucleon as a whole. 
Since many years the tensor charge is being calculated with steadily 
increasing accuracy by lattice QCD~\cite{Chen:2016utp}.
More recently, its connection with possible  novel tensor interactions at 
the TeV scale in neutron and nuclear $\beta$-decays and its possible 
contribution  to the neutron EDM have also been investigated~\cite{Bhattacharya:2016zcn}, 
and possible constraints on new physics beyond the standard mode have also 
been derived~\cite{Courtoy:2015haa}.
\begin{figure}
\begin{center}
\includegraphics[width=0.6\textwidth]{fig/gTcomp-explat-2016-06-09.pdf}
\end{center}
\vspace{-0.5cm}
\caption{ A summary plot showing the current estimates of $g_T^{u-d}$
  from Ref.~\protect\cite{Bhattacharya:2016zcn}.}
\label{fig:gT}
\end{figure}
The present knowledge on $g_T$ is well summarized in Fig. \ref{fig:gT}, 
from Ref.~\cite{Bhattacharya:2016zcn}. 
The huge difference between the accuracy of the extractions from the 
existing data and from the QCD lattice simulations is striking. 
Clearly more experimental data are needed. 
In the near future the only planned and approved experiments will run at 
JLab 12 [21,22], 
with very good statistics but $x>0.05$ and relatively small $Q^2$. 
In the longer term the planned EIC has the potential to carry on a very 
good programme scattering at high $\sqrt{s}$ electrons on transversely polarised 
protons or deuterons, but it is not yet on the real axis, and storing 
polarised deuterons is not yet in the core program.

We propose to measure during one full year, as soon as the LS2 will be 
over, SIDIS on a transversely polarised deuteron target in the M2 muon beam 
line. 
The polarised target will be reassembled at the end of the DVCS/SIDIS 
run, this 
fall, to be used for the Drell-Yan run of 2018, and will be left on the 
floor in Hall 888 for this new measurement. 
The main objective of the measurement is to improve (considerably) the 
accuracy of the extraction of $h_1^d$, but the precision of $h_1^u$ will also 
improve, by a factor 1.5-2 in the valence region ($x>0.1$), as will be shown 
in the next section. 
The \compass data will provide large $Q^2$ data in the $x$-range covered by 
JLab, which is very important to evaluate the size of the $Q^2$ evolution, 
and, most important, will provide lower-$x$ data (down to $x=0.005$) which 
are essential both to perform the integrals necessary to evaluate the tensor 
charges and to estimate the transversity of the sea quarks. 
Therefore they are complementary to the JLab 12 data. 
The phase space covered by the different experiments is shown in 
Fig. \ref{fig:xq2}.

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{fig/kinematics.pdf}
\end{center}
\vspace{-0.5cm}
\caption{$x-Q^2$ scatter plot for SIDIS experiments from Ref.~\protect\cite{Ye:2016prn}.} 
\label{fig:xq2}
\end{figure}


\subsubsection{Present COMPASS data and extrapolated errors}   

The transversity PDF is chiral-odd and thus not directly observable in 
inclusive deep inelastic lepton-nucleon scattering. 
In 1993 Collins suggested that it could be measured in SIDIS processes, where 
it appears coupled with another chiral-odd function~\cite{Bacchetta:2006tn}, 
which by now is known as ``Collins fragmentation function''  
$H^{\perp  h}_{1q}$. 
It is the chiral-odd transverse-spin dependent FF that describes the 
correlation of quark (q) transverse polarisation and hadron (h) transverse 
momentum. 
This mechanism leads to a left-right asymmetry in the distribution of hadrons 
produced in the fragmentation of transversely polarised quarks, which in 
SIDIS shows up as an azimuthal transverse spin asymmetry $A_{Coll}$ 
(the ``Collins asymmetry'') in the distribution of produced hadrons. 
At leading order this asymmetry can be written as
\begin{eqnarray}
 A_{Coll}(x,z, Q^2) 
= \frac{\sum_{q,\bar{q}} e_q^2 x h_1^q(x, Q^2)  \otimes H_{1q}^{\perp }(z, Q^2)}
{\sum_{q,\bar{q}} e_q^2 x f_1^q(x, Q^2) \otimes D_{1q}(z, Q^2)}
\label{collins2}
\end{eqnarray}
 where the sum is over all (anti)quark flavours, $D^h_q$ is the usual FF and 
$\otimes$ indicates the (different for numerator and denominator) convolutions 
over the intrinsic transverse momenta. 
The Collins effect shows up as a modulation 
$[1 + a_C sin(\phi_h + \phi_S - \pi)]$ in the hadron azimuthal distribution. 
Here the Collins angle $\Phi_C=\phi_h + \phi_S - \pi$ is the sum of the 
azimuthal angles of the hadron transverse momentum $\vec{p}_{hT}$ 
($\phi_h$) and of the spin direction of the target nucleon ($\phi_S$) 
with respect to the lepton scattering plane, in a reference system in which 
the z axis is the virtual-photon direction~\cite{Sivers:1989cc}. 
The amplitude of the modulation is $a_C = D_{NN} f P A_{Coll}$, where  
$D_{NN}$ is the transverse spin transfer coefficient from target quark to 
struck quark, $f$ the dilution factor of the target material, and $P$ is 
the proton (or deuteron) polarisation.
In Fig. \ref{fig:cpd}  the results for $A_{Coll}$ we have obtained~\cite{Adolph:2012sn}
from the 2010 data collected
using as target NH$_3$, a polarised proton target, are shown as a 
function of $x$ and compared to the results we obtained~\cite{Ageev:2006da}
from the deuteron runs of 2002-2003-2004, when as target we used $^6$LiD. 

\begin{figure}
\begin{center}
\includegraphics[width=0.8\textwidth]{fig/D1y_1h_0.pdf}
\end{center}
\vspace{-0.5cm}
\caption{ $A_{Coll}$  obtained from the 2010 data with the 
polarised proton NH$_3$ target as a 
function of $x$ (left plot)
compared to the results we obtained~\protect\cite{Ageev:2006da}
from the runs of 2002, 2003 and 2004 with polarised deuteron $^6$LiD target
(right plots). 
The red (black) points refer to positive (negative) hadrons.
The full points at -0.06 in the left plot show the extrapolated statistical
error from the proposed deuteron run (see text).}
\label{fig:cpd}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{fig/errors_d_p_0y.pdf}
\end{center}
\vspace{-0.5cm}
\caption{ Ratio of the  $A_{Coll}$ statistical uncertainties on 
deuteron and proton.} 
\label{fig:repd}
\end{figure}

It is clear that the accuracy of the data is considerably better for the 
proton run, in particular at large $x$, where the Collins asymmetry is large. 
In order to quantify this point, it is instructive to plot the ratio of the 
errors. 
In Fig. \ref{fig:repd} this ratio is shown 
again as a 
function of $x$.
In onder to understand this plot,
one has to remind that, for small asymmetries, the 
statistical error is given by 
\begin{eqnarray}
\sigma_A \simeq \frac{1}{fP} \frac{1}{\sqrt{N}} = \frac{1}{FOM} \frac{1}{\sqrt{N}}
\end{eqnarray}
where $N$ is the total number of hadrons and $FOM$ is the figure of merit
of the polarised target.
Using     $N_{d,h}=15.5 \cdot 10^6$ and $N_{p,h}=80 \cdot 10^6$ for the number
of hadrons collected
on p and d, and the known $FOM$ values for the two targets, one gets
\begin{eqnarray}
\frac{\sigma_{A_d}}{\sigma_{A_p}} = \frac{0.155 \cdot 0.80}{0.40 \cdot 0.50} 
\frac{\sqrt{80}}{\sqrt{15.5}} = 0.62 \cdot 2.3 = 1.4
\end{eqnarray}

At small $x$, where most of the events cluster, the ratio between the 
deuteron and the proton asymmetries is indeed constant, since the spectrometer 
acceptance was essentially the same in the two data taking, and its value 
is close to 1.4 (the small difference is due to the slightly different 
trigger mixture). 
Here the better $FOM$ of the deuteron target largely compensates the factor of 
5 in statistics in favour of the proton target. At large x on the contrary 
the ratio increases dramatically, reflecting the difference in acceptance 
of the PT magnet, which has a polar angle acceptance of 200 mrad as seen 
from the upstream end of the target, while in the earlier measurements with
 the $^6$LiD target we had utilized the SMC magnet, which has a polar angle 
acceptance of 70 mrad.

\subsubsection{Projected errors after 1 year of deuteron run}

{\em TO BE DETAILED IN THE NEXT VERSION}

Since target density and packing factors are essentially identical for 
$^6$LiD and NH$_3$, it can be safely assumed that in one year of deuteron 
run in the conditions of the 2010 proton run $80\cdot 10^6$ ``good'' events 
will be collected, so that the errors on the new deuteron asymmetries 
will be equal to the present errors for the 2010 proton asymmetries scaled 
by the ratio of the FOM, namely they will be smaller by a factor of 0.62. 
The projected errors for the deuteron asymmetries are 
also plotted in Fig. \ref{fig:cpd}, 
together with the existing deuteron and proton asymmetries. 
We neglect the systematic errors which were estimated to be at most 0.5 
times the statistical errors  in the 2010 data. 
Using the 2010 proton data and the projections of Fig.  \ref{fig:cpd} for the new deuteron 
data it is possible to extract the u- and d-quark transversity, and quantify 
the gain in statistical error in these fundamental PDF. 
To carry through this evaluation we have followed the procedure of Ref.~\cite{Martin:2014wua}, 
which allows a point by point extraction of transversity directly from the 
measured SIDIS and $e^+e^- \rightarrow hadrons$ asymmetries.

\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{fig/D1y_1h_1.pdf}
\end{center}
\vspace{-0.5cm}
\caption{Values 
of u$_v$-quark (left)  and d$_v$-quark (right)
transversity  extracted  from the existing p and d data (open points), and 
the corresponding error bars estimated using the existing 
p data and the new d data (closed points).} 
\label{fig:textr}
\end{figure}
The result of such extraction is given in Fig. \ref{fig:textr}, 
which shows both the values 
of transversity (open points) extracted  from the existing p and d data, and 
the corresponding error bars (closed points) estimated using the existing 
p data and the new d data. 
Also, Fig. \ref{fig:rtextr} gives the ratio, at each $x$ value, of the existing errors on 
the extracted transversities and the projected errors, taking the existing 
proton asymmetries from 2010 and the projected errors for the deuteron 
asymmetries obtained after 1 year of running. 
One can see that the gain in precision is quite good for the d-quark and 
important also for the u-quark.
\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{fig/D1y_1h_2.pdf}
\end{center}
\vspace{-0.5cm}
\caption{Ratio of the existing errors on 
the extracted transversities and the projected errors for u$_v$-quark 
(left)  and d$_v$-quark (right).} 
\label{fig:rtextr}
\end{figure}


\subsubsection{ Projections for the tensor charge}

{\em TO BE DETAILED IN THE NEXT VERSION}

In order to evaluate the tensor charge it is necessary to introduce a 
functional dependence for $h_1$. 
A popular choice is, neglecting the $Q^2$ dependence of $h_1$,
\begin{eqnarray}
x h_1^q(x) =  A x^{\alpha} (1-x)^{\beta} .
\end{eqnarray}
From a fit to the extracted values of $xh_1^u$ and $xh_1^d$ we get the 
90\% uncertainty bands as shown in Fig 7, and in turn the integrated values
\begin{eqnarray}
\delta u = xxx \pm xxx, \;\;\; 
\delta d = yyy \pm yyy, \;\;\;
g_T= \delta u - \delta d = zzz \pm zzz .
\end{eqnarray}
This estimate is meant only to propagate the statistical uncertainties 
from the measured PDF to to integrated tensor charges, but clearly for 
the extraction\\
- the high $x$ data from JLab will be necessary\\
- the $Q^2$ evolution must be taken into account.\\


\subsubsection{ Other measurements}

{\em TO BE DETAILED IN THE NEXT VERSION\\
di-hadron asymmetries,\\
Sivers and other TS asymmetries,\\
exclusive vector meson production}\\

\subsubsection{Experimental status of $\ell N \rightarrow \ell' h X$ on transversely polarised $N$}
\label{ssec:stdmuo.sidis.status}

\subsubsection{Extractions of transversity and Sivers PDFs}
\label{ssec:stdmuo.sidis.extraction}

\subsubsection{Projections for a one year run with the transversely polarised D target}
\label{ssec:stdmuo.sidis.projection}

\subsubsection{Competition}
\label{ssec:stdmuo.sidis.competition}


